DEVO: Depth-Event Camera Visual Odometry in Challenging Conditions

We present a novel real-time visual odometry framework for a stereo setup of a depth and high-resolution event camera. Our framework balances accuracy and robustness against computational efficiency towards strong performance in challenging scenarios. We extend conventional edge-based semi-dense visual odometry towards time-surface maps obtained from event streams. Semi-dense depth maps are generated by warping the corresponding depth values of the extrinsically calibrated depth camera. The tracking module updates the camera pose through efficient, geometric semi-dense 3D-2D edge alignment. Our approach is validated on both public and self-collected datasets captured under various conditions. We show that the proposed method performs comparable to state-of-the-art RGB-D camera-based alternatives in regular conditions, and eventually outperforms in challenging conditions such as high dynamics or low illumination.

==> compare_picture.tex <==
\global\long\def\figWidth{0.17\linewidth}
\begin{figure*}[!ht]
	\centering
    {\small
    \setlength{\tabcolsep}{2pt}
	\begin{tabular}{
	>{\centering\arraybackslash}m{0.5cm} 
	>{\centering\arraybackslash}m{\figWidth} 
	>{\centering\arraybackslash}m{\figWidth}
	>{\centering\arraybackslash}m{\figWidth} 
	>{\centering\arraybackslash}m{\figWidth}
	>{\centering\arraybackslash}m{\figWidth}}
		& Scene & Time Surface Map & Reprojection Map by~\cite{zhou2021event} & Reprojection Map (Ours)
		\\\addlinespace[1ex]

		\rotatebox{90}{\makecell{\indoorflying2{}}}
		&\includegraphics[width=\linewidth]{imgs/indoor2_rgb.png}
		&\includegraphics[width=\linewidth]{imgs/indoor2_ts.png}
		&\includegraphics[width=\linewidth]{imgs/indoor2_reproj_esvo.png}
		&\includegraphics[width=\linewidth]{imgs/indoor2_reproj_ours.png}
		\\%\addlinespace[1ex]

		\rotatebox{90}{\makecell{\indoorflying4{}}}
		&\includegraphics[width=\linewidth]{imgs/indoor4_rgb.png}
		&\includegraphics[width=\linewidth]{imgs/indoor4_ts.png}
		&\includegraphics[width=\linewidth]{imgs/indoor4_reproj_esvo.png}
		&\includegraphics[width=\linewidth]{imgs/indoor4_reproj_ours.png}
		\\%\addlinespace[1ex]

		\rotatebox{90}{\makecell{\outdoorday1{}}}
		&\includegraphics[width=\linewidth]{imgs/outdoor_rgb.png}
		&\includegraphics[width=\linewidth]{imgs/outdoor_ts.png}
		&\includegraphics[width=\linewidth]{imgs/outdoor_ts_esvo.png}
		&\includegraphics[width=\linewidth]{imgs/outdoor_reproj_ours.png}
		\\%\addlinespace[1ex]
	\end{tabular}
	}
	\caption{\label{fig:mapping:depthmaps-grid}\emph{Mapping}. 
	Qualitative comparison of mapping results (depth estimation) on several sequences using various stereo algorithms.
	The first column shows intensity frames from the DAVIS camera (not used, just for visualization).
	Columns 2 to 5 show inverse depth estimation results of \GTS~\cite{Ieng18fnins}, SGM~\cite{Hirschmuller08pami}, CopNet~\cite{Piatkowska17cvprw} and our method, respectively.
	Depth maps are color coded, from red (close) to blue (far) over a black background, 
	in the range \SIrange{0.55}{6.25}{\meter} for the top four rows (sequences from~\cite{Zhou18eccv})
	and the range \SIrange{1}{6.25}{\meter} for the bottom two rows (sequences from~\cite{Zhu18ral}).
	}
\end{figure*}

==> table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{p{4.2em}ccccp{.75em}cccp{.75em}cccp{.75em}p{4.2em}p{4.2em}p{4.2em}}
    \toprule
    　     & \multicolumn{1}{p{4.2em}}{　} & \multicolumn{3}{p{12.6em}}{Ours} & 　     & \multicolumn{3}{p{12.6em}}{Canny-VO} & 　     & \multicolumn{3}{p{12.6em}}{Kinect Fusion} & 　     & \multicolumn{3}{p{12.6em}}{ESVO} \\
\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}    \multicolumn{2}{p{8.4em}}{Sequence} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}    \multicolumn{2}{p{8.4em}}{\textit{cali\_bright\_fast}} & 3.73  & 2.03  & 23.67 & \multicolumn{1}{c}{} & 3.81  & 1.47  & 15.55 & \multicolumn{1}{c}{} & 3.74  & 1.81  & 15.34 & \multicolumn{1}{c}{} & -     & -     & - \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_bright\_mid}} & 1.44  & 1.77  & 16.9  & \multicolumn{1}{c}{} & 1.42  & 1.26  & 21.23 & \multicolumn{1}{c}{} & 1.35  & 1.77  & 19.22 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.58} & \multicolumn{1}{c}{1.48} & \multicolumn{1}{c}{55.41} \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_bright\_slow}} & 0.99  & 0.78  & 11.85 & \multicolumn{1}{c}{} & 1.03  & 0.59  & 7.16  & \multicolumn{1}{c}{} & 0.98  & 0.89  & 14.52 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.42} & \multicolumn{1}{c}{0.98} & \multicolumn{1}{c}{27.32} \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_darkish\_slow}} & 1.03  & 0.91  & 18.02 & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 1.02  & 0.93  & 11.34 & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_dim\_slow}} & 1.55  & 0.88  & 35.38 & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 1.62  & 0.82  & 9.05  & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_dark\_fast}} & 0.58  & 0.87  & 26.43 & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 0.63  & 0.92  & 12.61 & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_dark\_mid}} & 0.49  & 0.6   & 17.65 & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 0.54  & 0.59  & 12.89 & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_dark\_slow}} & 0.24  & \textit{0.31} & 9.85  & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 0.26  & 0.23  & 8.97  & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{cali\_hdr\_slow}} & 0.92  & 0.79  & 21.55 & \multicolumn{1}{c}{} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{p{4.2em}}{x} & \multicolumn{1}{c}{} & 0.95  & 0.71  & 11.1  & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{table\_bright\_fast}} & 1.5   & 2.42  & 46.37 & \multicolumn{1}{c}{} & 1.51  & 2.22  & 30.81 & \multicolumn{1}{c}{} & 1.38  & 2.75  & 27    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.81} & \multicolumn{1}{c}{2.75} & \multicolumn{1}{c}{149.32} \\
    \multicolumn{2}{p{8.4em}}{\textit{table\_bright\_mid}} & 1.16  & 1.53  & 27.83 & \multicolumn{1}{c}{} & 1.18  & 1.25  & 19.68 & \multicolumn{1}{c}{} & 1.1   & 1.79  & 21.71 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.65} & \multicolumn{1}{c}{1.88} & \multicolumn{1}{c}{68.9} \\
    \multicolumn{2}{p{8.4em}}{\textit{table\_bright\_slow}} & 0.63  & 1     & 19.5  & \multicolumn{1}{c}{} & 0.64  & 0.82  & 26.94 & \multicolumn{1}{c}{} & 0.59  & 1.15  & 22.48 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.38} & \multicolumn{1}{c}{1.28} & \multicolumn{1}{c}{34.74} \\
    \multicolumn{2}{p{8.4em}}{\textit{sofa\_bright\_fast}} & 2.6   & 2.3   & 30.22 & \multicolumn{1}{c}{} & 2.63  & 1.9   & 23.89 & \multicolumn{1}{c}{} & 2.6   & 3.64  & 27.79 & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{sofa\_bright\_mid}} & 5.28  & 4.02  & 13.4  & \multicolumn{1}{c}{} & 1.18  & 1.25  & 19.68 & \multicolumn{1}{c}{} & 3.13  & 7.62  & 71.5  & \multicolumn{1}{c}{} & x     & x     & x \\
    \multicolumn{2}{p{8.4em}}{\textit{sofa\_bright\_slow}} & 1.47  & 1.16  & 10.94 & 　     & 0.64  & 0.82  & 26.94 & 　     & 1.47  & 1.21  & 21.82 & 　     & x     & x     & x \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{cccccp{.75em}p{4.2em}p{4.2em}p{4.2em}p{.75em}p{4.2em}p{4.2em}p{4.2em}}
    \toprule
    \multicolumn{2}{p{8.4em}}{\textit{Frequency}} & \multicolumn{3}{p{12.6em}}{Ours} & 　     & \multicolumn{3}{p{12.6em}}{Canny-VO} & 　     & \multicolumn{3}{p{12.6em}}{Kinect Fusion} \\
\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{p{8.4em}}{\textit{High Table Fast}} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt  & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{c}{\textit{30}} & 1.5   & 2.42  & 46.37 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.51} & \multicolumn{1}{c}{2.22} & \multicolumn{1}{c}{30.81} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.37} & \multicolumn{1}{c}{2.75} & \multicolumn{1}{c}{27} \\
    \multicolumn{2}{c}{\textit{15}} & 2.92  & 4.86  & 46.7  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.96} & \multicolumn{1}{c}{4.46} & \multicolumn{1}{c}{29.11} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{3.04} & \multicolumn{1}{c}{8.36} & \multicolumn{1}{c}{37.99} \\
    \multicolumn{2}{c}{\textit{10}} & 4.26  & 7.32  & 47.92 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{4.65} & \multicolumn{1}{c}{6.55} & \multicolumn{1}{c}{34.68} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{4.83} & \multicolumn{1}{c}{17.33} & \multicolumn{1}{c}{66.78} \\
    \multicolumn{2}{c}{\textit{5}} & 7.73  & 14.73 & 57.89 & \multicolumn{1}{c}{} & x     & x     & x     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{9.01} & \multicolumn{1}{c}{26.86} & \multicolumn{1}{c}{55.09} \\
    \multicolumn{2}{c}{\textit{1}} & 18.58 & 49.16 & 76.04 & \multicolumn{1}{c}{} & x     & x     & x     & \multicolumn{1}{c}{} & x     & x     & x \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{p{8.4em}}{\textit{High Table Medium}} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt  & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{c}{\textit{30}} & 1.16  & 1.53  & 27.83 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.18} & \multicolumn{1}{c}{1.25} & \multicolumn{1}{c}{19.68} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.1} & \multicolumn{1}{c}{1.79} & \multicolumn{1}{c}{21.71} \\
    \multicolumn{2}{c}{\textit{15}} & 2.29  & 3.01  & 24.2  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.34} & \multicolumn{1}{c}{2.48} & \multicolumn{1}{c}{20.08} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.17} & \multicolumn{1}{c}{3.56} & \multicolumn{1}{c}{21.31} \\
    \multicolumn{2}{c}{\textit{10}} & 3.39  & 4.51  & 21.46 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{3.49} & \multicolumn{1}{c}{3.7} & \multicolumn{1}{c}{20.34} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{3.2} & \multicolumn{1}{c}{5.58} & \multicolumn{1}{c}{58.73} \\
    \multicolumn{2}{c}{\textit{5}} & 6.55  & 9.2   & 21.55 & \multicolumn{1}{c}{} & x     & x     & x     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{7.16} & \multicolumn{1}{c}{15.8} & \multicolumn{1}{c}{37.07} \\
    \multicolumn{2}{c}{\textit{1}} & 18.46 & 35.24 & 51.93 & \multicolumn{1}{c}{} & x     & x     & x     & \multicolumn{1}{c}{} & x     & x     & x \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{p{8.4em}}{\textit{High Table Slow}} & \multicolumn{1}{p{4.2em}}{RPEr} & \multicolumn{1}{p{4.2em}}{RPEt} & \multicolumn{1}{p{4.2em}}{ATEt} & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt  & \multicolumn{1}{c}{} & RPEr  & RPEt  & ATEt \\
\cmidrule{1-5}\cmidrule{7-9}\cmidrule{11-13}    \multicolumn{2}{c}{\textit{30}} & 0.63  & 1     & 19.5  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.64} & \multicolumn{1}{c}{0.82} & \multicolumn{1}{c}{26.94} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.59} & \multicolumn{1}{c}{1.15} & \multicolumn{1}{c}{22.48} \\
    \multicolumn{2}{c}{\textit{15}} & 1.21  & 1.97  & 18.44 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.24} & \multicolumn{1}{c}{1.65} & \multicolumn{1}{c}{26.01} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.13} & \multicolumn{1}{c}{2.29} & \multicolumn{1}{c}{22.22} \\
    \multicolumn{2}{c}{\textit{10}} & 1.76  & 2.98  & 18.46 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.82} & \multicolumn{1}{c}{2.46} & \multicolumn{1}{c}{26.32} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.66} & \multicolumn{1}{c}{3.41} & \multicolumn{1}{c}{22.1} \\
    \multicolumn{2}{c}{\textit{5}} & 3.28  & 6.09  & 17.61 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{3.71} & \multicolumn{1}{c}{5.54} & \multicolumn{1}{c}{27.97} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{3.17} & \multicolumn{1}{c}{16.57} & \multicolumn{1}{c}{120.77} \\
    \multicolumn{2}{c}{\textit{1}} & 10.66 & 31.15 & 37.88 & 　     & x     & x     & x     & 　     & x     & x     & x \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

